Looking Beyond IoCs: Automatically Extracting Attack Patterns from External CTI

Public and commercial organizations extensively share cyberthreat intelligence (CTI) to prepare systems to defend against existing and emerging cyberattacks. However, traditional CTI has primarily focused on tracking known threat indicators such as IP addresses and domain names, which may not provide long-term value in defending against evolving attacks. To address this challenge, we propose to use more robust threat intelligence signals called attack patterns. LADDER is a knowledge extraction framework that can extract text-based attack patterns from CTI reports at scale. The framework characterizes attack patterns by capturing the phases of an attack in Android and enterprise networks and systematically maps them to the MITRE ATT\&CK pattern framework. LADDER can be used by security analysts to determine the presence of attack vectors related to existing and emerging threats, enabling them to prepare defenses proactively. We also present several use cases to demonstrate the application of LADDER in real-world scenarios. Finally, we provide a new, open-access benchmark malware dataset to train future cyberthreat intelligence models.

==> sections/approach.tex <==

% TODO: A subgraph for all cerberus nodes
%---------------------------------------%
\section{Approach Overview - \textsf{LADDER}}\label{framework}
%---------------------------------------%
The main idea of our proposed framework \textsf{LADDER} is that gathering past threat intelligence, like attack patterns, can train a threat intelligence model for (a) detecting semantically similar attack patterns occurring in threat analysis reports and (b) inferring attack tactic or technique for an emerging attack vector based on the available information. 
% Our team of researchers analyzed many malware attack pattern steps and concluded that most could be mapped to the MITRE ATT\&CK pattern framework. While each step's granular, low-level information is detailed, all attack patterns can be abstracted to a high-level definition.

% \textcolor{blue}{Analyzing a subset of 80 attack patterns collected from different CTIs, we could map most of them to a unique MITRE ID. However, in some cases, there may be some ambiguity between different attack pattern descriptions, or some attack patterns may not be yet listed for the platform (more details in Section \ref{sec:usecase}). Regardless, attack patterns provide a more abstract detail of attack steps compared to low-level granular descriptions. }

% and mapped to the descriptions from MITRE ATT\&CK.
Additionally, \textsf{LADDER} captures additional information, such as locations, indicators of compromise (IoCs), and system information which can help identify the similarity between different malware and threat actors.
\par
In this section, we provide a summary of the \textsf{LADDER} framework and modules. \textsf{LADDER} comprises four modules for using threat intelligence from CTI when they are structured and analyzed by a knowledge graph-based system. \textsf{LADDER} aggregates unstructured threat and attack information from diverse CTI sources and provides actionable analysis to security analysts (see Figure \ref{fig:ladder}). Once trained and ready for use, a security analyst submits a corpus of unstructured threat information into \textsf{LADDER}. The trained system returns inferred intelligence like most machine learning models. However, instead of simply classifying the ingested data, \textsf{LADDER} returns classes along with matching instances. The predefined classes are - \textsf{Malware, Malware Type, Application, Operating System, Organization, Person, Time, Threat Actor, Location, Attack Pattern}. Nine of the ten classes return a list of classes and their respective instances found in the CTI. 
%The Attack Pattern class can return more than one instance of attack patterns as it infers the next tactic or technique for the malware whose CTI was ingested. 
See Figure \ref{fig:ladder} for a high-level view of the framework and its various modules. We describe each of these in detail next.
\begin{figure*}
\centering
\includegraphics[width=1\textwidth,height=.33\textwidth]{figures/framework.png}
\caption{Proposed framework: \textsf{LADDER} and the five component modules. (a) Extracts CTI using crawlers, (b) Pre-processes and prepares for entity and relationship extraction, (c) generates data in the form of triples, (d) creates a knowledge graph by combining the triples and uses graph embedding methods to pack every triple's properties into a vector with smaller dimensions, and (e) returns instances when to queried by the analyst. (a)-(d) are training step, (e) is inference step.}
\label{fig:ladder}
\end{figure*}


%\par
%\noindent
%{\tt{``In June 2019, ThreatFabric analysts found a new Android malware, dubbed “Cerberus”, being rented out on underground forums. Along with the standard payload and string obfuscation, Cerberus uses device accelerometer sensor to implement a simple pedometer that is used to measure movements of the victim. When the malware is first started on the device it will begin by hiding its icon from the application drawer. Then it will ask for the accessibility service privilege. Most Android banking Trojans use overlay attacks to trick the victim into providing their personal information and Cerberus is no exception. It mostly targets French and US banking apps, especially banking users in Italy. Package name of latest Cerberus sample com.uxlgtsvfdc.zipvwntdy.”}}
%\newline

% \begin{figure}[H]
% \centering
% \includegraphics[width=.49\textwidth]{figures/CTIsnap.png}
% \caption{An excerpt from Threatpost report on Cerberus trojan}
% \label{fig:CTIsnap}
% \end{figure}

\subsection{Cyberthreat Intelligence (CTI)}\label{sec:CTI}
CTI is usually available in the form of after-action reports \cite{Piplai2020CreatingCK}, unstructured blogs, security bulletins \cite{MSFTSecurityBulletin}, and technical reports. A standard approach to examining CTI reports involves (a) perusing the most prevalent techniques, trends, and threats observed by the author(s), (b) detecting, mitigating, and simulating specific threats and techniques, and (c) mapping ideas, guidance, and priorities to their security measures and general strategy. Analysts can track down and defend against known attacks using IoCs. More importantly, information like tactics, techniques, and procedures written in semantic format is assembled to characterize a threat attack for analysis and future predictions. We design a high-performance web crawler (details in appendix) that scrapes, collects, and stores over 90k unstructured threat report from 2010 to 2022. These threat reports explain the attack behavior of malware and APTs targeted at various platforms such as windows, Linux, Android, and iOS operating systems. Out of these, over 12K reports had descriptions for mobile malware.

\subsection{Concepts of threat intelligence}\label{sec:concepts}
We extract threat intelligence concepts as a triple, $\langle entity_{head}-relationship-entity_{tail}\rangle$. Also known as a semantic triple, it codifies a statement in a threat report about the malware in an RDF format, $\langle subject, predicate, object\rangle$ expressions. The triple entity is representative of one of ten classes from CTI reports-- \textsf{Malware, Malware Type, Application, Operating System, Organization, Person, Time, Threat Actor, Location, Attack Pattern}. These triples aggregate in the threat intelligence knowledge graph, transforming the multi-modal open-access CTI into a structured format. Security analysts can use this graph to systematically \textit{query} known threats and emerging threats and forecast trends and attack patterns using evidence in the form of existing knowledge in the graph. 
%This evidence can be either in the form of an unstructured CTI source or a triple, $\langle entity_{head},relationship,entity_{tail}\rangle$. 
The concepts are detailed in the Appendix.

% \begin{table}[!h]
% %% increase table row spacing, adjust to taste
% \centering
% \caption{A few triples (entity, relationship, entity) corresponding to the open-access CTI report for malware Cerberus.}
% \label{table:triple_list}
% %% Some packages, such as MDW tools, offer better commands for making tables
% %% than the plain LaTeX2e tabular which is used here.
% \resizebox{0.50\textwidth}{!}
% {
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{$entity_{head}$} (concept) & relationship & \textbf{$entity_{tail}$} (concept)\\
% \hline
% Cerberus(class: Malware) & targets & Android(class: OS)\\
% %Cerberus(class: Malware) & discovered in & June, 2019(class: Time)\\
% Cerberus(class: Malware) & targets & Spain(class: Location)\\
% Cerberus(class: Malware) & uses & Calculadora de Moneda(class: Application)\\
% Cerberus(class: Malware) & uses & Hide application icon(class: Attack Pattern)\\
% Cerberus(class: Malware) & uses & Steal victim's bank-account credentials(class: Attack Pattern)\\
% Cerberus(class: Malware) & uses & Bypass security measures(class: Attack Pattern)\\
% \hline
% \end{tabular}
% }
% \end{table}

\subsection{Generating Threat Intelligence Graph}
Open-access CTI reports are passed %are ingested 
into information extraction models pre-trained from triples collected from hand-annotated CTI reports. Hence, the extraction of relevant entities and asserting the relationship between entities are the key procedures to generate a graph. Traditionally information graphs were constructed using pre-existing databases constructed by domain experts. However, for cybersecurity, we can utilize information extraction techniques and machine learning to collect facts from unstructured text sources and populate the graph.

\subsection{Inferring Attack Patterns}
The information extraction module also comprises an algorithm we propose-- \textsf{TTPClassifier} that automates attack pattern extraction from CTI reports. In Figure \ref{fig:Cerberus}(b), \textsf{TTPClassifier} extracts all known malware attack behaviors and guides us to a list of attack behaviors not seen before. The triple formed from this attack behavior is \textsf{$\langle Cerberus, uses,conduct\ covert\ surveillance\rangle$}. 
\par
Inferring attack patterns using \textsf{LADDER} works as follows: (a) \textbf{Training: }The knowledge graph comprising attack behaviors, classes, and relationships of all known, existing, and dormant malware are extracted from CTI sources using \textsf{TTPClassifier} and other information extraction models. Additionally, \textsf{TTPClassifier} also maps these behaviors to MITRE ATT\&CK pattern IDs. %(see Table \ref{table:mitre}.
(b) \textbf{Inferring: } When inferring new threat intelligence from an emerging threat, the security analyst queries the knowledge graph by inputting a triple, where the tail entity is missing. The \textsf{LADDER} framework infers all blank tail entities, including attack behaviors and all other classes, along with a confidence score. 
%We describe the technical details in Section \ref{infoExtract}.
\par
In \textsf{TTPClassifier}, the attack behavior is mapped to an existing MITRE ATT\&CK technique. MITRE ATT\&CK provides a comprehensive list of threat tactics and techniques based on real-world malware attacks. 
%It is foundational to developing defenses against known threats to enterprise and mobile platforms. 
The list consists of a detailed description of different cybercriminals' attack techniques. It also provides corresponding mitigation measures for each attack pattern technique. For example, a total of 66 attack techniques are listed for mobile malware. See Table \ref{tab:MITREattack} in the Appendix for an exhaustive list of attack IDs and corresponding descriptions. 
% Once \textsf{LADDER} extracts attack patterns from unstructured text, it can map them to the standard MITRE's techniques using a mapping algorithm. This automates the process of understanding threats and obtaining mitigation measures from CTI.

% \begin{table}[H]
% \centering
% \scriptsize
% \caption{MITRE ATT\&CK Techniques for Mobile Malware}
% \label{table:mitre}
% %\resizebox{0.36\textwidth}{!}
% {%
% \begin{tabular}{|l|l|}
% \hline
% \textbf{Technique ID} & \textbf{Description}                                                  \\ \hline
% T1626          & Abuse Elevation Control Mechanism                               \\ \hline
% T1517 & Access Notifications \\ \hline
% T1640   & Account Access Removal                       \\ \hline
% T1638      & Adversary-in-the-Middle                            \\ \hline
% T1429 & Audio Capture                        \\ \hline
% T1616     & Call Control                         \\ \hline
% T1641           & Data Manipulation    \\ \hline
% T1456             & Drive by Compromise \\ \hline
% T1407             & Download New Code at Runtime \\ \hline

% \end{tabular}%
% }
% \end{table}

